Neutrino Direct Simulation Monte Carlo: Accurate modeling of out-of-equilibrium decaying cosmological relics

We consider nonstandard cosmologies in which decaying relics inject energy at MeV temperatures, driving neutrinos out of equilibrium. The subsequent neutrino evolution shapes predictions for the cosmic radiation density and primordial light element abundances. Earlier work introduced Neutrino Direct Simulation Monte Carlo ($\nu$DSMC), which describes neutrino transport through Monte Carlo sampling of particle interactions. Here, we extend this method by jointly evolving the relic population, neutrino spectra, electromagnetic plasma, and cosmic expansion, and coupling this evolution to Big Bang nucleosynthesis. The framework includes direct and inverse decays of the relic, neutrino flavor conversion, quantum statistics, and pion production by energetic neutrinos. To reveal the physical impact of these effects and independently test $\nu$DSMC, we compare several approaches to neutrino evolution across a range of nonstandard cosmological scenarios. We find excellent agreement with independent solutions of quantum kinetic or quasi-classical Boltzmann equations. Compared with these calculations, $\nu$DSMC includes a broader range of physical processes and is substantially faster for strongly nonthermal neutrino populations. This makes broad, robust parameter scans for nonstandard cosmologies practical. We show that when departures from thermal equilibrium are large, approximations that average over neutrino momenta can give qualitatively incorrect predictions, including the wrong sign of the change in the effective number of neutrino species and substantially incorrect primordial nuclear abundances. We conclude that the extended $\nu$DSMC framework enables reliable cosmological tests of new physics by following neutrino thermalization and its observable consequences.

==> header_DSMC_new.tex <==
\RequirePackage[colorlinks=true
,urlcolor=black
,anchorcolor=black
,citecolor=black
,filecolor=black
,linkcolor=black
,menucolor=black
,linktocpage=true
,pdfproducer=medialab
,pdfa=true
]{hyperref}

\usepackage{eso-pic}
\newcommand{\reportnum}[2]{
  \AddToShipoutPictureBG*{%
    \AtPageUpperLeft{%
      \hspace{0.75\paperwidth}%
      \raisebox{#1\baselineskip}{%
        \makebox[0pt][l]{\textnormal{#2}}
  }}}%
}

\usepackage{amsmath,amssymb,amsthm,amsfonts,mathtools}
\usepackage{graphicx}
\usepackage{color}
\usepackage{xcolor}
\colorlet{BLUE}{black}
\colorlet{RED}{black}
\colorlet{MAGENTA}{magenta}
\colorlet{PURPLE}{purple}
\usepackage{multirow}
\usepackage{comment}
\usepackage{xspace}
\usepackage{enumitem}
\usepackage{cleveref}
\usepackage{slashed, bm}
\usepackage[normalem]{ulem}
\usepackage{scalerel}
\usepackage{textgreek}
\usepackage{physics}

\setlist[description]{leftmargin=0.3cm}
\setlist[itemize]{leftmargin=0.5cm}

% Keep each footnote intact across columns, pages, and widetext transitions.
\interfootnotelinepenalty=10000

\newcommand{\be}{\begin{equation} \begin{aligned}}
\newcommand{\ee}{\end{aligned} \end{equation}}
\newcommand{\beqa}{\begin{eqnarray}}
\newcommand{\eeqa}{\end{eqnarray}}

\newcommand{\mX}{\ensuremath{m_{X}}\xspace}
\newcommand{\tX}{\ensuremath{\tau_{X}}\xspace}
\newcommand{\Treh}{\ensuremath{T_{\rm reh}}\xspace}
\newcommand{\neff}{\ensuremath{N_{\rm eff}}\xspace}
\newcommand{\dH}{\ensuremath{\text{D}/\text{H}|_{\rm P}}\xspace}
\newcommand{\mev}{\ensuremath{\,{\rm MeV}}\xspace}
\newcommand{\yp}{\ensuremath{Y_{\rm P}}\xspace}
\newcommand{\gev}{\ensuremath{\,{\rm GeV}}\xspace}
\newcommand{\tev}{\ensuremath{\,{\rm TeV}}\xspace}
\newcommand{\s}{\ensuremath{\,{\rm s}}\xspace}
\newcommand{\dneff}{\ensuremath{\Delta N_{\text{eff}}}\xspace}
\newcommand{\dyp}{\ensuremath{\Delta Y_{\rm P}}\xspace}
\newcommand{\ddhfive}{\ensuremath{\Delta({\rm D/H})_5}\xspace}
\newcommand{\neffsbbn}{\ensuremath{N_{\rm eff}^{\rm SBBN}}\xspace}
\newcommand{\ypsbbn}{\ensuremath{Y_{\rm P}^{\rm SBBN}}\xspace}
\newcommand{\dhsbbn}{\ensuremath{({\rm D/H})_{\rm SBBN}}\xspace}
\newcommand{\pn}{\ensuremath{p\leftrightarrow n}\xspace}

% Semantic typography for the calculation and scenario names used in prose.
% Lowercase input is intentional: it produces genuine small capitals.
\DeclareRobustCommand{\nudsmc}{\ensuremath{\nu}\textsc{dsmc}\xspace}
% Section headings are set in capitals; use a full-height, bold rendering there
% instead of the smaller prose small caps.
\DeclareRobustCommand{\nudsmcheading}{\ensuremath{\nu}\mbox{DSMC}\xspace}
\DeclareRobustCommand{\thermalmethod}{\textsc{Thermal}\xspace}
\DeclareRobustCommand{\qcbemethod}{\textsc{qcbe}\xspace}
\DeclareRobustCommand{\qkemethod}{\textsc{qke}\xspace}
\DeclareRobustCommand{\setupname}[1]{\textit{Scenario~#1}}
\pdfstringdefDisableCommands{%
  \def\nudsmc{nuDSMC}%
  \def\nudsmcheading{nuDSMC}%
  \def\thermalmethod{Thermal}%
  \def\qcbemethod{QCBE}%
  \def\qkemethod{QKE}%
  \def\setupname#1{Scenario #1}%
}

\def\figureautorefname~#1\null{Fig.\,#1\null}
\def\tableautorefname~#1\null{Tab.\,#1\null}
\renewcommand{\sectionautorefname}{Sec.}
\renewcommand{\subsectionautorefname}{Sec.}
\def\equationautorefname~#1\null{Eq.\,(#1)\null}

% General symbols
\newcommand{\im}{\mathrm{i}}
\newcommand{\diff}{\mathrm{d}}
\newcommand{\eg}{{e.\,g.}~}
\newcommand{\ie}{{i.\,e.}~}
\newcommand{\equivalent}{\simeq}
\newcommand{\br}{\mathrm{BR}}

\newcommand{\Tspl}{\ensuremath{T_{\rm split}}\xspace}
\newcommand{\Tini}{\ensuremath{T_{\rm ini}}\xspace}

\newcommand{\ab}{\text{ab}}
\newcommand{\iab}{\text{ab}^{-1}}
\newcommand{\fb}{\text{fb}}
\newcommand{\ifb}{\text{fb}^{-1}}
\newcommand{\ipb}{\text{pb}^{-1}}

\newcommand{\nm}{\text{nm}}
\newcommand{\micm}{\mu\text{m}}
\newcommand{\mm}{\text{mm}}
\newcommand{\cm}{\text{cm}}
\newcommand{\m}{\text{m}}
\newcommand{\km}{\text{km}}
\newcommand{\MeV}{\ensuremath{\text{ MeV}}\xspace}


%comments
\RequirePackage[normalem]{ulem} 
\newcommand{\changed}[2]{#2}
%\newcommand{\changed}[2]{#2}

\crefname{section}{Sec.}{Secs.}
\crefname{figure}{Fig.}{Figs.}
\crefname{table}{Table}{Tables}
\crefname{equation}{Eq.}{Eqs.}
\crefname{appendix}{Appendix}{Appendices}

%Ref Style
\bibliographystyle{utphys}

